Semi-Supervised Learning on Graphs Based on Local Label Distributions

Most approaches that tackle the problem of node classification consider nodes to be similar, if they have shared neighbors or are close to each other in the graph. Recent methods for attributed graphs additionally take attributes of neighboring nodes into account. We argue that the class labels of the neighbors bear important information and considering them helps to improve classification quality. Two nodes which are similar based on class labels in their neighborhood do not need to be close-by in the graph and may even belong to different connected components. In this work, we propose a novel approach for the semi-supervised node classification. Precisely, we propose a new node embedding which is based on the class labels in the local neighborhood of a node. We show that this is a different setting from attribute-based embeddings and thus, we propose a new method to learn label-based node embeddings which can mirror a variety of relations between the class labels of neighboring nodes. Our experimental evaluation demonstrates that our new methods can significantly improve the prediction quality on real world data sets.

==> with_comments/conclusion_.tex <==
% !TEX root = main.tex
\vspace{-1ex}
\section{Conclusion}
\label{sec:conclusion}

In this paper, we have introduced a novel label-based approach for semi-supervised node classification. In particular, our method aggregates labels from local neighborhoods using APPR. Most existing approaches consider nodes to be similar, if they are closely related in the graph. Methods for attributed graphs additionally take attributes of the neighboring nodes into account. In contrast, our method can relate nodes even if they are not close-by in the graph and makes more effective use of the labels provided for training to improve the classification quality for graphs with and without node attributes. It is further applicable to nodes unseen during training. The results of our experiments on various real-work datasets demonstrate that local label distributions are able to significantly improve classification results in the multiclass and multilabel setting. Our model is even competitive with state-of-the-art models, which take node attributes into consideration. In a first experiment on multilabel datasets, we were already able to significantly boost the performance by using a simple combination of our model with node embeddings.

For future work, we plan to address the problem of selecting a suitable teleportation parameter $\alpha$.
The $\alpha$ parameter controls the extend of the considered local neighborhood and often has a significant impact on the prediction quality. Performing a grid search to determine a good parameter value is a time consuming task. Furthermore, for different classes varying teleportation parameters might yield the best results.
 
We also aim at further improving the prediction accuracy by further investigating how to effectively combine label-based features with different other kinds of other features, such as node attributes, edge attributes or node embeddings in a semi-supervised model.
Our approach could also be extended to solve additional graph learning tasks, such as link prediction or identification of nodes with unexpected labels for detecting labeling errors or outlier nodes.

\vspace{-1ex}

%In this paper, we introduce a novel label-based approach to semi-supervised learning in graph-structured data. In contrast to existing methods relying on graph structure or node attributes, our approach leverages the rich information provided by the label distribution in the graph. This enables our methods to learn how groups, defined by labels, appear in the graph and how they depend on each other locally. Our method learns corresponding node representations by efficiently extracting label distributions in relevant neighborhoods of varying size defined by Approximate Personalized PageRank and additionally learns an optimal combination of the resulting distributions. Experiments on text classification benchmark datasets demonstrate that our method is able to effectively leverage label information to improve node classification compared to related methods relying only on the graph structure. Further results on the same graph datasets with additional node attributes suggest that our method is competitive with state-of-the-art methods for attributed graphs, and that the relevance of label information for node classification is comparable to that of node attributes. Additional experiments on multi-label classification on a biological and a social network are promising, but reveal potential for future work, since most of the classes in the considered datasets appear very locally in the graph and some of them are very small. Also, different labels are not necessarily correlated. Better results could be achieved with more adaptable architectures. Another extension that we plan to address in our future work is a more elaborate combination of labels with classical node features to consider correlations between these two types of information and to capture more interesting group patterns.


==> with_comments/experiments_.tex <==
%!TEX root = ./main.tex
\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.45\columnwidth}
        \includegraphics[width=\textwidth]{figures/single_alpha_figures/cora_noFeat_microf1_boxplot.pdf}
        \vspace{-7ex}
        \caption{Micro F$_1$ scores for \textit{Cora}.}
        \label{fig:cora}
    \end{subfigure}
    %
    \begin{subfigure}[t]{0.45\columnwidth}
        \includegraphics[width=\textwidth]{figures/single_alpha_figures/citeseer_noFeat_microf1_boxplot.pdf}
        \vspace{-7ex}
        \caption{Micro F$_1$ scores for \textit{CiteSeer}.}
        \label{fig:citeseer}
    \end{subfigure}
    %
    \begin{subfigure}[t]{0.45\columnwidth}
        \includegraphics[width=\textwidth]{figures/single_alpha_figures/pubmed_noFeat_microf1_boxplot.pdf}
        \vspace{-7ex}
        \caption{Micro F$_1$ scores for \textit{Pubmed}.}
        \label{fig:pubmed}
    \end{subfigure}
    %\vspace{-2ex}
    \caption{Micro F$_1$ scores for the three benchmark data sets.}\label{fig:acc}
    %\vspace{-4ex}
\end{figure*}

%\vspace{-1ex}
\section{Evaluation}\label{sec:experiments}
We evaluate our approach by performing node-label prediction and compare the quality in terms of micro F$_1$ score %, which corresponds to accuracy 
for multiclass prediction tasks, respectively micro F$_1$ and macro F$_1$ scores for multilabel prediction tasks, against state-of-the-art methods.% \footnote{The code will be published upon acceptance}

For both tasks, we compare our model against the following approaches:
\begin{itemize}
\item \textit{Adj}: a baseline approach which learns node embeddings only based on the information contained in the adjacency matrix
%\item \textit{Feat}: a baseline approach which predicts node labels only based on the node features without considering the underlying graph structure (borrowed from \cite{yang2016revisiting})
%\item GCN variants: we use several variants of the graph convolution network (GCN) model proposed in \cite{kipf2016semi}
%\begin{itemize}
\item \textit{GCN$_1$\_only\_L}: a GCN which applies convolution on label matrix $\mathbf{Y}$. We use one convolution layer on the adjacency matrix without self-links, followed by a dense output layer\footnote{\label{foot:why_one_layer_gcn}See \ref{subsec:motivation} for the explanation why only one convolution layer makes sense}
%\item \textit{GCN$_1$+L}: also one convolution and one dense layer as in previous model. This model combines node attributes and label informations.
%%To combine the node attributes preprocessed adjacency matrix as in Kipf et al. is used. Labels from the neighborhood are collected with the preprocessed adjacency matrix without self links.
%The convolution layer has the form: $ReLU(\:[\hat{A}F,\hat{A}_{w/o\_self-links}Y_{train}]\:W)$, where $\hat{A}$ and $\hat{A}_{w/o\_self-links}$ are as in Kipf et al. preprocessed  adjacency matrices (with and  without self links) and $[\cdot, \cdot]$ is concatenation operation.
%\item \textit{GCN$_2$}: the standard 2-layer GCN as published by Kipf et al.
\item \textit{noFeat GCN$_2$}: the standard 2-layer GCN as published by Kipf et al. \cite{kipf2016semi} without using the node attributes
%\end{itemize}
%\item \textit{Chebychev$_3$}: the spectral convolution method which uses chebychev filters as presented in \cite{NIPS2016_6081}; as in \cite{kipf2016semi} we also use 3rd order chebychev filters
\item \textit{DeepWalk}: the DeepWalk model as proposed in \cite{perozzi2014deepwalk}
\item \textit{node2vec}: the node2vec model as proposed in \cite{grover2016node2vec}
%\item \textit{Planetoid-T}: the semi-supervised Planetoid framework which uses feature information as proposed in \cite{yang2016revisiting}
\item \textit{Planetoid-G}: the Planetoid variant which does not use attribute information \cite{yang2016revisiting}
\footnote{Unless stated differently we use for all competitors the parameter settings as suggested by the corresponding authors. Except for minor adaptations, e.g., to include label information in the one layer GCN models or to make the Planetoid models applicable for multilabel prediciton tasks, we use the original implementations as published by the correpsonding authors.}
\end{itemize}

Our model is denoted as \textit{LD} (short for \underline{L}abel \underline{D}istribution). For these experiments we train a simple feed-forward neural network which takes the label distribution based representations as input and retrieves class probabilities as output.


%In particular, we compare our models against (1) \textit{GCN-noFeat}: a variant of the graph convolutional model as proposed in \cite{kipf2016semi} that does not incorporate the node feature matrix to learn the embeddings, (2) \textit{Planetoid-G}: the model as proposed in \cite{yang2016revisiting}, that is a Planetoid variant derived from the transductive model but also does not consider the feature matrix to learn the embeddings, (3) \textit{DeepWalk} embeddings \cite{perozzi2014deepwalk}, (4) \textit{node2vec} embeddings \cite{grover2016node2vec} and (5) a baseline approach that tries to predict the nodes' label only based on the adjacency matrix of the underlying graph. We do not include comparison with \textit{struct2vec}, because we could not run it even for our smallest graph. We stopped experiment after two weeks.
%Furthermore, to demonstrate the power of our approach, we also compare against the variants of GCN and Planetoid that also use information captured within the feature matrix (denoted as \textit{GCN}, resp. \textit{Planetoid-T}).
%We borrow the baseline approach from \cite{yang2016revisiting} which predicts only based on the node features without considering the underlying graph structure (denoted as \textit{Feat}). We also compare against the technique presented in \cite{NIPS2016_6081}, a spectral convolution method which uses Chebyshev filters. For our experiments we used 3rd order Chebyshev filters (\textit{Chebyshev3}).

%We denote our models as \textit{LD-CONCAT} for fully connected combination (Equation \ref{eq:fully_connected} in Section \ref{sec:method}), \textit{LD-INDP} for Equation \ref{eq:indep_diff_weights},  \textit{LD-INDP-SHARED} if the weights are shared (Equation \ref{eq:shared_comb}) and finally \textit{LD-AVG} for weighted average (Equation \ref{eq:simple_weights}).

Note that we omit the comparison to label propagation \cite{zhu2003semi} since Yang et al. already showed that the \textit{Planetoid} model outperforms this approach \cite{yang2016revisiting}.

\vspace{-1ex}
\subsection{Multiclass Prediciton}

\subsubsection{Experimental Setup}\label{sec:setup}
For the multiclass label prediciton task we use the following three text classification benchmark graph datasets \cite{sen2008collective, namata2012query}:
\begin{itemize}
\item \textsc{Cora}. The Cora dataset contains 2'708 publications from seven categories in the area of ML. The citation graph consists of 2'708 nodes, 5'278 edges, 1'433 attributes and 7 classes.
\item \textsc{CiteSeer}. The CiteSeer dataset contains 3'264 publications from six categories in the area of CS. The citation graph consists of 3'264 nodes, 4'536 edges, 3'703 attributes and 6 classes.
\item \textsc{Pubmed}. The Pubmed dataset contains 19'717 publications which are related to diabetes and categorized into 3 classes. The citation graph consists of 19'717 nodes, 44'324 edges, 500 attributes and 3 classes.
\end{itemize}
\noindent For each graph, documents are denoted as nodes and undirected links between documents represent citation relationships. If node attributes are applied, bag-of-words representations are used as attribute vectors for each document.

We split the data as suggested in \cite{yang2016revisiting}, i.e., for labeled data our training sets contain 20 randomly selected instances per class, the test sets consist of 1'000 instances, and the validation sets contain 500 instances for each method. The remaining instances are used as unlabeled data. For comparison we use the prediction micro F$_1$ scores which we collected over 10 different data splits.

Since the numbers of iterations for sampling the graph contexts and the label contexts for \textit{Planetoid} are suggested only for the \textit{CiteSeer} data set, we adapted these values relative to the number of nodes for each graph. For \textit{node2vec}, we perform grid searches over the hyperparameters $p$ and $q$ with $p,q \in \lbrace 0.25, 0.5, 1.0, 2.0, 4.0\rbrace$ and use window size 10 as proposed by the authors. %Considering our models, we perform grid searches over the set $\lbrace 4, 8, 16, 32\rbrace$ for the number of hidden units \red{evgeniy: $output\_per\_input$?}.
For all models except \textit{Planetoid} unless otherwise noted, we use one hidden layer with 16 neurons and regularization, learning rate and training procedure as in \cite{kipf2016semi}.  Considering our model, we use $\alpha \in \lbrace 0.1, 0.2, \ldots, 0.9\rbrace$ as values for the teleportation parameter and $\epsilon = 1e^{-5}$ as approximation threshold to compute the APPR vectors for each node.

We present results computed on the test sets for the best performing hyperparameters. The best performing hyperparameters for all models are determined by using the validation sets.


%We present our results for the best performing $\alpha$ parameter, which is determined based on validation set.

%\vspace{-1ex}
\subsubsection{Results}\label{sec:results}
%\begin{table}[t]  %[htb]
%\begin{center}
%\begin{adjustbox}{max width=\columnwidth}
%  \begin{tabular}{  | r | c  c  c | }
%  \hline
%    \multirow{2}{*}{\textsc{Method}} & \multicolumn{3}{c }{\textsc{Dataset}} \\ %\cline{2-4}
%     & \textsc{Cora} & \textsc{CiteSeer} & \textsc{Pubmed} \\ \hline
%    \textsc{Adj} & 0.521 & 0.330 & 0.398 \\ \hline
%    \textsc{GCN-noFeat} & 0.657 & 0.459 & 0.382 \\ \hline
%    \textsc{Planetoid-G} & 0.691 & 0.493 &  0.664 \\ \hline
%    \textsc{DeepWalk} & 0.706 & 0.512 & 0.760 \\ \hline
%    %\textsc{GraRep} & 0.696 & 0.517 & 0.733 \\ \hline
%    \textsc{node2vec} & 0.724 & 0.529 & 0.785 \\ \hline
%    %\textsc{Single Alpha} & 0.849 & 0.586 & 0.798 \\ \hline
%    \textsc{Ld-Concat} & 0.841 & 0.581 & 0.794 \\ \hline
%    \textsc{Ld-Indp} & 0.844 & 0.589 & 0.796 \\ \hline
%    \textsc{Ld-Indp-Shared} & 0.843 & 0.585 & 0.796 \\ \hline
%    \textsc{Ld-avg} & 0.831 & 0.582 & 0.784 \\ \hline
%    %\textsc{Combined Alphas Attention} & 0.846 & 0.591 & 0.788 \\ \hline
%    %\textsc{Combined Shared Weights with Binary Alpha Identification} & 0.841 & 0.617 & 0.795 \\ \hline
%    %\textsc{Combined Shared Weights with Continuous Alpha Identification} & 0.840 & 0.616 & 0.799 \\ \hline
%    %\textsc{Gated Continuous Alpha} & 0.842 & 0.586 & 0.799 \\ \hline
%    %\textsc{Gated Binary Alpha} & 0.842 & 0.581 & 0.802 \\ \hline
%    %\textsc{Bahdanau Attention on Continous Alpha Per Dim} & 0.847 & 0.586 & 0.785 \\ \hline
%    %\textsc{Bahdanau Attention on Binary Alpha Per Dim} & 0.847 & 0.601 & 0.793 \\ \hline
%    %\textsc{Bahdanau Attention on Continous Alpha} & 0.849 & 0.593 & 0.791 \\ \hline
%    %\textsc{Bahdanau Attention on Binary Alpha} & 0.849 & 0.596 & 0.796 \\ \hline
%    %\textsc{Attention on Continous Alpha} & 0.846 & 0.577 & 0.784 \\ \hline
%    %\textsc{Attention on Binary Alpha} & 0.850 & 0.592 & 0.791 \\
%  \end{tabular}
%  \end{adjustbox}
%  \end{center}
%  \caption{Accuracy values for each method and the three considered text classification benchmark graph data sets when ignoring the node features.}
%  \label{tab:nofeat}
%\end{table}
Figure~\ref{fig:acc} shows boxplots depicting the micro F$_1$ scores we achieved for the multiclass prediction task for each considered model on the \textit{Cora}, \textit{CiteSeer} and \textit{Pubmed} networks.

The baseline approach \textit{GCN$_1$\_only\_L}, i.e., the one layer GCN model which only uses the label distributions of the neighboring nodes to predict a node's label, shows worst results among the considered models. However, these scores are still promising that the labels may improve the task of learning ``good'' representations. The baseline method which considers the corresponding rows of the adjacency matrix as node representations, i.e., \textit{Adj}, achieves slightly better results for all three datasets. For the \textit{GCN} and \textit{Planetoid} models that do not make recourse to attribute information, i.e., \textit{noFeat GCN$_2$}, resp. \textit{Planetoid-G}, the retrieved micro F$_1$ values are slightly lower than the ones achieved by \textit{DeepWalk} and \textit{node2vec}.
Our model improve the results produced by \textit{node2vec}, which means that the label distributions are indeed a useful source of information, although the baseline \textit{GCN$_1$\_only\_L} shows, especially for \textit{Pubmed}, rather poor results. This may be reasoned by the fact that this model only considers the label distribution of a very local neighborhood (in fact one hop neighbors). However, collecting the label distribution from a more spacious neighborhood gives a significant boost in terms of prediction accuracy. Indeed the best results for the \textit{LD} approach are reached for $\alpha = 0.1$, which corresponds to a rather spacious neighborhood exploration.
%Moreover, for all datasets, our models perform similarly, which shows that even simple models with shared weights are able to match the performance of more complex models.


%Following our intuition, this also means that different nodes indeed benefit from different neighborhood extensions which ultimately depends on the distribution of the corresponding class labels.


%The results of the experiments for which we ignored the feature vectors are shown in Table~\ref{tab:nofeat}. The baseline method, i.e., \textit{Adj}, which considers the corresponding rows of the adjacency matrix as node representations shows rather poor results and are clearly worst in case of Cora and CiteSeer. Since the \textit{GCN} and \textit{Planetoid} models cannot make recourse to feature information in this case, the retrieved accuracy values are slightly lower than the ones given from \textit{DeepWalk}, \textit{GraRep} and \textit{node2vec}. However, our models improve the results produced by \textit{node2vec}. On Cora we even achieve more than 17\% gain of accuracy. the
%For all datasets, the fourth of our proposed models, i.e., the model which learns different weights for different neighborhoods, performs best.
%For all datasets, our models perform similarly, which shows that even simple models with shared weights are able to match the performance of more complex models.
%Following our intuition, this also means that different nodes indeed benefit from different neighborhood extensions which ultimately depends on the distribution of the corresponding class labels.

%Overall, the model which takes a single PPR matrix as input performs best. This is due to the fact that there seems to exist kind of optima in the extension of considered neighborhoods, which in turn means that there are (potentially a few) $\alpha$ values for which the PPR vectors capture the label distribution within the neighborhood of the considered node best. The rest of our approaches somehow combine the PPR matrices gathered from different values for $\alpha$, but as we used the same set of $\alpha$ values for all experiments, the combinations are, unless the label distributions of single classes are extremely heterogeneous, not likely to be better than the model which uses only the PPR matrix of the $\alpha$ value  from our set, that approaches best the average of ``best neighborhood extension'' over all nodes.

%\subsubsection{Comparison to models that use features}
%Considering the models that do use feature information, the comparison to the performance of our models is not so monotonous. For \textit{Cora}, where feature information and label information seem to be comparable helpful for the node classification task (we draw this conclusion from the fact that the baseline approaches \textit{Feat} and \textit{GCN$_1$\_only\_L} achieve similar accuracies) our models show similar performance than the state-of-the-art two-layer \textit{GCN} model, i.e., \textit{GCN$_2$}, but outperform other competitors that use features, e.g., \textit{Chebychev$_3$} or \textit{Planetoid-T}. For \textit{CiteSeer}, \textit{Feat} shows a better performance than \textit{GCN$_1$\_only\_L} and following our intuition, the established models which use features also perform better than the models which only include label information. Nevertheless, for \textit{Pubmed} our models show very similar performance as the feature-including models, although our baseline model for the influence of label information performs much worse than the \textit{Feat} model. This is reasoned by the fact that the \textit{GCN$_1$\_only\_L} only uses the label information from one-hop neighbors to predict a node's label. Due to using a combination of label information gathered from very local neighborhoods (coming from APPR matrices calculated with large values for $\alpha$; in this case $\alpha=0.9$), and label information collected from relatively wide neighborhoods (coming from APPR matrices which were calculated with very small values for $\alpha$; in this experiment $\alpha=0.01$) for our models, they still achieve very good results. We discuss this in more detail in Section~\ref{sec:discussion}.
%\begin{table}[t]  %[htb]
%\begin{center}
%  \begin{tabular}{ | r | c  c  c | }
%  \hline
%    \multirow{2}{*}{\textsc{Method}} & \multicolumn{3}{c |}{\textsc{Dataset}} \\ %\cline{2-4}
%     & \textsc{Cora} & \textsc{CiteSeer} & \textsc{Pubmed} \\ \hline
%    \textsc{Feat} & 0.591 & 0.600 & 0.699 \\ \hline
%    \textsc{GCN} & 0.815 & 0.679 & 0.789 \\ \hline
%    \textsc{Chebyshev3} & 0.800 & 0.693 & 0.648 \\ \hline
%    \textsc{Planetoid-T} & 0.757 & 0.629 & 0.757 \\ \hline
%    \textsc{Best of our models} & 0.844 & 0.589 & 0.796 \\ \hline
%  \end{tabular}
%  \end{center}
%  \caption{Accuracy values for each method and the three considered text classification benchmark graph data sets when considering the node features.}
%  \label{tab:withfeat}
%\end{table}
%Interestingly, our models even outperform the state-of-the-art methodologies that explicitly make use of the node features, c.f., Table~\ref{tab:withfeat}. Although the \textit{GCN} and \textit{Planetoid} versions that incorporate the node features significantly improve the accuracy values over their featureless counterparts, the final results of our models on Cora and Pubmed are still better. On CiteSeer, the baseline approach, \textit{Feat}, works already better than our models. This indicates that incorporating the node features is likely to improve the outcome for the node classification task. Thus, the three competitors, of course, also benefit from the features and achieve better scores.
\vspace{-1ex}
\subsection{Multilabel Classification}
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.45\columnwidth}
        \includegraphics[width=\textwidth]{figures/single_alpha_figures/blogcatalog_single_alpha_microf1_boxplot.pdf}
        \vspace{-6ex}
        \caption{Micro F$_1$ scores for \textit{BlogCatalog}.}
        \vspace{-0ex}
        \label{fig:blogcatalog_micro}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.45\columnwidth}
        \includegraphics[width=\textwidth]{figures/single_alpha_figures/blogcatalog_single_alpha_macro_f1_boxplot.pdf}
        \vspace{-6ex}
        \caption{Macro F$_1$ scores for \textit{BlogCatalog}.}
        \label{fig:blogcatalog_macro}
    \end{subfigure}
    %\vspace{-2ex}
    \caption{Micro F$_1$ and macro F$_1$ for \textit{BlogCatalog}.}\label{fig:blogcatalog}
    %\vspace{-1ex}
\end{figure}

%\begin{table}[t]  %[htb]
%\begin{center}
%\begin{adjustbox}{max width=\columnwidth}
%  \begin{tabular}{  r | c  c  c  c }
%    \multirow{3}{*}{\textsc{Method}} & \multicolumn{4}{c }{\textsc{Dataset}} \\ %\cline{2-4}
%     & \multicolumn{2}{c }{\textsc{PPI}} & \multicolumn{2}{c }{\textsc{BlogCatalog}} \\ \cline{2-5}
%     & micro-F$_1$ & macro-F$_1$ & micro-F$_1$ & macro-F$_1$ \\ \hline
%    \textsc{Adj} & 0.078 & 0.042 & 0.158 & 0.033 \\ \hline
%    \textsc{GCN-noFeat} & 0.014 & 0.012 & 0.0 & 0.0 \\ \hline
%    \textsc{Planetoid-G} & 0.108 & 0.060 &  - & - \\ \hline
%    \textsc{DeepWalk} & 0.146 & 0.107 & 0.237 & 0.124 \\ \hline
%    \textsc{GraRep} & 0.157 & 0.120 & 0.255 & 0.139 \\ \hline
%    \textsc{node2vec} & 0.151 & 0.109 & 0.246 & 0.129 \\ \hline
%    \textsc{Single Alpha} & 0.108 & 0.055 & 0.185 & 0.064 \\ \hline
%    \textsc{Combined Alphas Simple Weights} & 0.111 & 0.065 & 0.189 & 0.082 \\ \hline
%    \textsc{Combined Alphas Concat} & 0.111 & 0.063 & 0.191 & 0.083 \\ \hline
%    %\textsc{Combined Alphas Attention} & 0.846 & 0.591 & 0.788 \\ \hline
%    \textsc{Combined Shared Weights} & 0.109 & 0.055 & 0.194 & 0.079 \\ \hline
%    %\textsc{Combined Shared Weights with Binary Alpha Identification} & 0.841 & 0.617 & 0.795 \\ \hline
%    %\textsc{Combined Shared Weights with Continuous Alpha Identification} & 0.840 & 0.616 & 0.799 \\ \hline
%    \textsc{Combined Different Weights} & 0.111 & 0.059 & 0.202 & 0.085 \\
%    %\textsc{Gated Continuous Alpha} & 0.842 & 0.586 & 0.799 \\ \hline
%    %\textsc{Gated Binary Alpha} & 0.842 & 0.581 & 0.802 \\ \hline
%    %\textsc{Bahdanau Attention on Continous Alpha Per Dim} & 0.847 & 0.586 & 0.785 \\ \hline
%    %\textsc{Bahdanau Attention on Binary Alpha Per Dim} & 0.847 & 0.601 & 0.793 \\ \hline
%    %\textsc{Bahdanau Attention on Continous Alpha} & 0.849 & 0.593 & 0.791 \\ \hline
%    %\textsc{Bahdanau Attention on Binary Alpha} & 0.849 & 0.596 & 0.796 \\ \hline
%    %\textsc{Attention on Continous Alpha} & 0.846 & 0.577 & 0.784 \\ \hline
%    %\textsc{Attention on Binary Alpha} & 0.850 & 0.592 & 0.791 \\
%  \end{tabular}
%  \end{adjustbox}
%  \end{center}
%  \caption{Micro-F$_1$ and Macro-F$_1$ scores for each method resulting from multilabel classifications on the two considered graph data sets. Training volume is 10\%.}
%  \label{tab:ten}
%\end{table}

\subsubsection{Experimental Setup}
We also perform multilabel node classifications on the following two multilabel networks:

\begin{itemize}
\item \textsc{BlogCatalog} \cite{tang2009relational}. This is a social network graph where each of the 10,312 nodes corresponds to a user and the 333,983 edges represent the friendship relationships between bloggers. 39 different interest groups provide the labels.
\item \textsc{IMDb Germany}. This dataset is taken from \cite{faerman2017lasagne}. It consists of 32,732 nodes, 1,175,364 edges and 27 labels. Each node represents an actor/actress who played in a German movie. Edges connect actors/actresses that were in a cast together and the node labels represent the genres that the corresponding actor/actress played.
\end{itemize}
Since the fraction of positive instances is relatively small for most of the classes, we use weighted cross-entropy as loss function. Therefore, the loss caused by erroneously classified positive instances is weighted higher. We use weight 10 in all our experiments. For the same reason we report micro F$_1$ and macro F$_1$ score metrics to measure the quality of the considered methods.
We compare our model to the featureless models that we already used for the multiclass experiments \footnote{To adapt the \textit{Planetoid-G} implementation for multilabel classification, we use a \textit{sigmoid} activation function at the output layer and also slightly changed the embedding learning step. Entities that are used as context and have the same labels as the node itself are sampled from all classes to which the node belongs to.}.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.45\columnwidth}
        \includegraphics[width=\textwidth]{figures/single_alpha_figures/imdb_germany_single_alpha_microf1_boxplot.pdf}
        \vspace{-6ex}
        \caption{Micro F$_1$ scores for \textit{IMDb Germany}.}
        \label{fig:imdb_micro}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.45\columnwidth}
        \includegraphics[width=\textwidth]{figures/single_alpha_figures/imdb_germany_single_alpha_macro_f1_boxplot.pdf}
        \vspace{-6ex}
        \caption{Macro F$_1$ scores for \textit{IMDb Germany}.}
        \label{fig:imdb_macro}
    \end{subfigure}
    %\vspace{-2ex}
    \caption{Micro F$_1$ and macro F$_1$ for \textit{IMDb Germany}.}\label{fig:imdb}
    %\vspace{-1ex}
\end{figure}
%We also adapted the \textit{Planetoid-G} implementation for multilabel classification. Besides a $sigmoid$ activation function at the output layer, we also changed the embedding learning step. Entities with same labels used as context are sampled from all classes to which the object belongs to.

%The results can be seen in Table~\ref{tab:seventy}.
We split the data into training, validation and test set so that 70\% of all nodes were used for training, 10\% for validation and 20\% of the data were used to test the model. Note that we could not use stratified sampling splits for these experiments since we optimize for all classes simultaneously instead of using one-vs-rest classifiers \footnote{That is why our results for \textit{node2vec} and \textit{DeepWalk} on the BlogCatalog network are slightly worse than reported in \cite{grover2016node2vec}}. The hyperparameter setting is as described above. For this set of experiments we ran each model, except for \textit{Planetoid-G}, 10 times on five different data splits. Due to the long runtime of \textit{Planetoid-G} we trained this model only three times on two data splits.

%\begin{table}[t]  %[htb]
%\begin{center}
%\begin{adjustbox}{max width=\columnwidth}
%  \begin{tabular}{ | r | c  c  c  c | }
%  \hline
%    \multirow{3}{*}{\textsc{Method}} & \multicolumn{4}{c |}{\textsc{Dataset}} \\ %\cline{2-4}
%     & \multicolumn{2}{c }{\textsc{PPI}} & \multicolumn{2}{c |}{\textsc{BlogCatalog}} \\ \cline{2-5}
%     & micro-F$_1$ & macro-F$_1$ & micro-F$_1$ & macro-F$_1$ \\ \hline
%    \textsc{Adj} & 0.026 & 0.015 & 0.136 & 0.008 \\ \hline
%    \textsc{GCN-noFeat} & 0.009 & 0.007 & 0.0 & 0.0 \\ \hline
%    \textsc{Planetoid-G} & 0.069 & 0.067 &  0.091 & 0.064 \\ \hline
%    \textsc{DeepWalk} & 0.189 & 0.136 & 0.268 & 0.084 \\ \hline
%    %\textsc{GraRep} & 0.193 & 0.152 & 0.344 & 0.123 \\ \hline
%    \textsc{node2vec} & 0.198 & 0.142 & 0.279 & 0.085 \\ \hline
%    %\textsc{Single Alpha} & 0.175 & 0.107 & 0.161 & 0.047 \\ \hline
%    \textsc{LD-CONCAT} & 0.173 & 0.108 & 0.220 & 0.063 \\ \hline
%    %\textsc{Combined Alphas Attention} & 0.846 & 0.591 & 0.788 \\ \hline
%    %\textsc{Combined Shared Weights with Binary Alpha Identification} & 0.841 & 0.617 & 0.795 \\ \hline
%    %\textsc{Combined Shared Weights with Continuous Alpha Identification} & 0.840 & 0.616 & 0.799 \\ \hline
%    \textsc{LD-INDP} & 0.180 & 0.124 & 0.306 & 0.123 \\ \hline
%    \textsc{LD-INDP-SHARED} & 0.173 & 0.117 & 0.302 & 0.120 \\ \hline
%    \textsc{LD-AVG} & 0.176 & 0.110 & 0.182 & 0.049 \\ \hline
%    %\textsc{Gated Continuous Alpha} & 0.842 & 0.586 & 0.799 \\ \hline
%    %\textsc{Gated Binary Alpha} & 0.842 & 0.581 & 0.802 \\ \hline
%    %\textsc{Bahdanau Attention on Continous Alpha Per Dim} & 0.847 & 0.586 & 0.785 \\ \hline
%    %\textsc{Bahdanau Attention on Binary Alpha Per Dim} & 0.847 & 0.601 & 0.793 \\ \hline
%    %\textsc{Bahdanau Attention on Continous Alpha} & 0.849 & 0.593 & 0.791 \\ \hline
%    %\textsc{Bahdanau Attention on Binary Alpha} & 0.849 & 0.596 & 0.796 \\ \hline
%    %\textsc{Attention on Continous Alpha} & 0.846 & 0.577 & 0.784 \\ \hline
%    %\textsc{Attention on Binary Alpha} & 0.850 & 0.592 & 0.791 \\
%  \end{tabular}
%  \end{adjustbox}
%  \end{center}
%  \caption{Micro-F$_1$ and Macro-F$_1$ scores for each method resulting from multilabel classifications on the two considered graph data sets. Training volume is 70\%.}
%  \label{tab:seventy}
%\end{table}
\begin{figure*}[htb!]
    \centering
    \begin{subfigure}[t]{0.45\columnwidth}
        \includegraphics[width=\textwidth]{figures/single_alpha_figures/cora_withFeat_microf1_boxplot.pdf}
        \vspace{-7ex}
        \caption{Micro F$_1$ scores for \textit{Cora}.}
        \label{fig:cora_feat}
    \end{subfigure}
    %
    \begin{subfigure}[t]{0.45\columnwidth}
        \includegraphics[width=\textwidth]{figures/single_alpha_figures/citeseer_withFeat_microf1_boxplot.pdf}
        \vspace{-7ex}
        \caption{Micro F$_1$ scores for \textit{CiteSeer}.}
        \label{fig:citeseer_feat}
    \end{subfigure}
    %
    \begin{subfigure}[t]{0.45\columnwidth}
        \includegraphics[width=\textwidth]{figures/single_alpha_figures/pubmed_withFeat_microf1_boxplot.pdf}
        \vspace{-7ex}
        \caption{Micro F$_1$ scores for \textit{Pubmed}.}
        \label{fig:pubmed_feat}
    \end{subfigure}
    %\vspace{-2ex}
    \caption{Comparison against attribute-based methods: micro F$_1$ scores for the three benchmark data sets.}\label{fig:acc_feat}
    %\vspace{-2ex}
\end{figure*}
\subsubsection{Results}
The results for the \textit{BlogCatalog} graph are shown in Figure~\ref{fig:blogcatalog}. For this network, only using the label information from the direct neighborhood of a node is not useful to infer its labels, c.f., \textit{GCN$_1$\_only\_L}. However, incorporating the label distribution of somewhat larger neighborhoods as for our model (again, we also use the APPR matrix calculated for small values of $\alpha$ to determine the label distribution in neighborhoods that span more than 1-hop neighbors) seems to improve the results for the prediciton task significantly. In fact, our model achieves similar, but slightly worse performance than \textit{node2vec} and \textit{DeepWalk}. Given these results, we also combined the node embeddings based on local label distributions with embeddings that capture structural properties. To capture the structural properties we select a very simple approach: we multiply an embedding matrix with the preprocessed adjacency matrix as in Kipf et al. \cite{kipf2016semi}. The embedding matrix is randomly initialized. Note that the structural similarity is defined via direct neighbors. The resulting representation is concatenated with the hidden layer of the \textit{LD} model and the rest of the \textit{LD} model remains the same. The embedding weights are learned jointly with rest of the model.
%The resulting representation is concatenated with the representations from the \textit{LD} model. The concatenated vector is given as input into a feed-forward neural network, and the embedding matrix is learned. The model can be formalized as follows,
%$$\text{\textit{LD+EMB}}=concat(AW_{emb},R_{LD}),$$ with $A$ denoting the adjacency matrix, $W_{emb}$ denoting the embedding matrix and $R_{LD}$ describing the representations retrieved from the $LD$ model.
Having a look at the scores for the resulting model, denoted as \textit{LD+EMB}, this combination further improves the outcome of the prediction.

For the \textit{IMDb Germany} network, for which the results can be seen in Figure~\ref{fig:imdb}%\footnote{The results for Planetoid-G on IMDb Germany are still running and are displayed for only one split. We will adapt the plots for the camera ready version.}
, the labels of even very local neighborhoods are already very expressive. Recalling how this network is constructed, we can expect the latter fact and also the superior performance of our model over the two random walk based methods. Particularly noteworthy for this network is the gain of accuracy that the combination of information from both sources, label distribution and structural properties, achieves.

%\vspace{-1ex}
\subsection{Comparison to Attribute-Based Methods}
To show the power of incorporating label information into the generation process for node embeddings, we also compare our model against the following state-of-the-art attribute-based methods:
\begin{itemize}
\item \textit{Feat}: a baseline approach which predicts node labels only based on the node attributes without considering the underlying graph structure (borrowed from \cite{yang2016revisiting})
\item \textit{GCN$_2$}: the standard 2-layer GCN as published in \cite{kipf2016semi}
\item \textit{Chebychev$_3$}: the spectral convolution method which uses chebychev filters as presented in \cite{NIPS2016_6081}; as in \cite{kipf2016semi} we also use 3rd order chebychev filters
\item \textit{Planetoid-T}: the semi-supervised Planetoid framework which uses attribute information as proposed in \cite{yang2016revisiting}
\end{itemize}
For this set of experiments, we again perform multiclass prediciton on the three benchmark text classification datasets and report the prediction accuracy in terms of micro F$_1$ scores to measure the quality of the retrieved node representations. Note that in contrast to the competitors, our model still does not make use of the node attribute information.
The results are depicted in Figure~\ref{fig:acc_feat} and clearly show that our model can definitely compete with the attribute-based methods and hence is a powerful alternative in cases when no node attributes are present.

%\vspace{-1ex}
\subsection{Impact of the $\alpha$ Parameter}
\begin{figure*}[htb!]
    \centering
    \begin{subfigure}[t]{0.45\columnwidth}
        \includegraphics[width=\textwidth]{figures/single_alpha_figures/cora_diff_alphas_microf1_boxplot.pdf}
        \vspace{-5ex}
        \caption{Micro F$_1$ scores for \textit{Cora}.}
        \label{fig:cora_feat}
    \end{subfigure}
    %
    \begin{subfigure}[t]{0.45\columnwidth}
        \includegraphics[width=\textwidth]{figures/single_alpha_figures/citeseer_diff_alphas_microf1_boxplot.pdf}
        \vspace{-5ex}
        \caption{Micro F$_1$ scores for \textit{CiteSeer}.}
        \label{fig:citeseer_feat}
    \end{subfigure}
    %
    \begin{subfigure}[t]{0.45\columnwidth}
        \includegraphics[width=\textwidth]{figures/single_alpha_figures/pubmed_diff_alphas_microf1_boxplot.pdf}
        \vspace{-5ex}
        \caption{Micro F$_1$ scores for \textit{Pubmed}.}
        \label{fig:pubmed_feat}
    \end{subfigure}
    %\vspace{-2ex}
    \caption{Micro F$_1$ scores for the three benchmark data sets when considering different locality levels for node neighborhoods.}\label{fig:diff_alphas}
    %\vspace{-2ex}
\end{figure*}

Figure~\ref{fig:diff_alphas} depicts the micro F$_1$ scores achieved for different values of the teleportation parameter $\alpha$ on the three benchmark datasets. As can be seen, particularly for the \textit{Pubmed} network, the model is quite sensitive to the choice of this parameter. Recall that the teleportation parameter determines how far the neighborhood of each node shall be taken into consideration to get the label distributions for each node. Therefore it might make sense to set the $\alpha$ parameter to a small value so that more labels are collected which in turn leads to a more accurate estimation of the local label distribution. On the other hand, this may not hold in every scenario, for instance if the distribution of classes is heterogeneous, i.e., some classes may only appear in areas of the graph where classes are concentrated locally, while other classes may appear in areas where many classes are mixed even within local neighborhoods. An interesting direction for future work is therefore to optimize for some ``good'' $\alpha$ value in a data-driven manner. This may be done either by pre-defining a set of different values of $\alpha$ and approaching for the best of these, or by trying to optimize for some ``good'' $\alpha$ value during the learning procedure. Also, the underlying task, e.g., node classification, may benefit from finding ``good'' values of $\alpha$ for each node individually rather than relying on a global solution.


==> with_comments/introduction_.tex <==
% !TEX root = main.tex
%\vspace{-3ex}
\section{Introduction}
\label{sec:intro}

Graphs are the most general way to represent structured data. In general, a set of entities with some given pairwise relationships between them can be modeled as a graph $G=(V,E)$ with a corresponding node set $V$ and an edge set $E \subseteq V \times V$. Real-world examples of graph-structured data are abundant and include social networks, co-citation networks or biological networks.

In addition to the graph structure, further attribute information may be provided for the entities described by the graph nodes. In an attributed graph, each node $v_i \in V$ is associated with an attribute vector $f_i \in \R^d$. For instance, social network users might be enriched with personal information or documents in a co-citation network might be described by bag-of-words vectors. The increasing relevance of graph-structured data has been accompanied by an increased interest in learning algorithms which can leverage underlying graph structure to make accurate predictions for the modeled entities.

An important semi-supervised learning task on graphs is node classification, where each node $v_i \in V$ can be associated with a set of class labels (simply referred to as labels in the following) represented by a label vector $y_i \in \{0,1\}^l$ where $l$ is the number of possible labels. Given a set of already labeled nodes in a graph, the goal is to predict new likely labels for unlabeled nodes. The task is semi-supervised in the sense that connectivity information about the whole graph is available and at least some of the class labels are already known. In the case of attributed graphs, attributes of all nodes can additionally be used for prediction, including those of the unlabeled nodes in the graph. Important applications include recommendation in social networks, where the node labels represent user interests, or document classification in co-citation networks, where the node labels indicate associated fields of research.

%Important applications of this problem include recommendation in social networks, where the nodes of the graph correspond to the users, the edges model friendship or following relations, and the labels of a user represent her interests. The ... Other common applications include ...
Approaches for node classification on graphs may employ additional node attributes or operate on the graph structure alone. We will refer to these approaches as \emph{attribute-based} and \emph{connectivity-based} approaches, respectively.
%Based on the success of deep learning in a multitude of applications, recent activity in the field exhibits a strong focus on generalizing such models to graph-structured domains.
Among the most successful connectivity-based methods are node embedding techniques \cite{perozzi2014deepwalk, grover2016node2vec, tang2015line, faerman2017lasagne, cao2015grarep, wang2016structural, ribeiro2017struc2vec, hamilton2017inductive, bojchevski2017deep, kipf2016variational}.
%The main idea is to learn a feature vector $x_i \in \R^k$ for each node $v_i \in V$ which represents $v_i$'s local connectivity. Node labels are then predicted from the learned feature vectors using a (multi-label) classifier. The underlying assumption is that nodes which are closely related in the graph, should have similar labels which is commonly referred to as homophily \cite{mcpherson2001birds}.
An underlying assumption of these techniques is that nodes which are closely connected in the graph, should have similar labels, which is commonly referred to as homophily \cite{mcpherson2001birds}.
Our method does not rely on the homophily assumption, but is still able to relate close-by nodes. Furthermore, unlike most node embedding techniques our new approach can be used to classify nodes unseen during training.
In the attribute-based setting the graph structure can be incorporated in different ways, for instance by using regularization \cite{zhu2003semi, zhou2004learning, belkin2006manifold, weston2012deep}, combining attributes with node embeddings \cite{yang2016revisiting}, or aggregating them over local neighborhoods \cite{DBLP:journals/corr/BrunaZSL13,DBLP:journals/corr/HenaffBL15, NIPS2016_6081, kipf2016semi, DBLP:journals/corr/AtwoodT15, DBLP:journals/corr/MontiBMRSB16, DBLP:journals/corr/LevieMBB17,simonovsky2017dynamic,velivckovic2017graph}. While regularization-based methods rely on the homophily assumption and most of them are not able to classify instances unseen during training, all other methods focus on node attributes.
%In the attribute-based setting, the feature vector $x_i$ corresponds to the attribute vector $f_i$. The graph structure can be incorporated in different ways. For instance, \emph{Laplacian regularization} \cite{zhu2003semi, belkin2006manifold, weston2012deep} implements the homophily assumption by adding a regularizer to the prediction loss. In the \emph{Planetoid} framework \cite{yang2016revisiting}, both, node embeddings and node attributes, act as features used for prediction. \emph{Graph convolution} models \cite{DBLP:journals/corr/BrunaZSL13,DBLP:journals/corr/HenaffBL15, NIPS2016_6081, kipf2016semi, DBLP:journals/corr/AtwoodT15, DBLP:journals/corr/MontiBMRSB16, DBLP:journals/corr/LevieMBB17,simonovsky2017dynamic,velivckovic2017graph} aggregate node attributes over local neighborhoods with spatially localized filters, similar to classical convolutional networks on images \cite{lecun1989backpropagation}.
In addition to connectivity and node attributes, the labels available during training further provide valuable information that is in general complementary to connectivity and attribute features, and are useful to improve classification.
In general learning tasks on independent and identically distributed (iid) data, labels indicate that an observation is sampled from a particular distribution. However, in a graph we have non-iid data and thus, the labels of connected objects allow for a novel use of label information which has not been exploited before for learning graph embeddings.

% While any classification model with separated training and inference phases naturally uses labels as targets during training, to the best of our knowledge, no existing model makes effective use of the labels of connected nodes as additional input features for prediction.

In this paper, we propose a \emph{label-based} approach to learn a node embedding which allows for more accurate node classifications. The main idea of our approach is that there often exists a correlation between the labels of a node and the distribution of labels in its local neighborhood. Thus, considering the local label distribution when computing a node embedding can exploit this correlation to improve the descriptiveness of the learned embedding.
In Figure \ref{fig:example}, we illustrate this for a typical case for which the label of a node is determined by the labels of neighboring nodes and not by node attributes or connectivity. As an additional example, the function of a protein can be expected to correlate strongly with the functions of interacting proteins.
%Aggregating labels over local neighborhoods further allows for dealing with sparse training labels.
As mentioned above, we assume that the labels of at least some of the neighboring nodes are known for each new node with unknown labels. In the majority of applications, this is realistic because new nodes usually connect to already known parts of the network. For instance, new papers usually cite established articles and new members of a social network will usually already know multiple friends in the network to connect to.

\begin{figure}
\centering
\includegraphics[width=0.65\columnwidth]{figures/paper_motivation_label_distribution.jpg}
%\vspace{-3ex}
\caption{Consider a communication network with nodes labeled according to their device type (user, server, database, printer). Assume the labels for the database and printer nodes in the right connected component are unknown while the remaining labels are provided. Further node attributes are not given. We can observe that the roles of printers and databases are clearly defined by the labels of their neighboring nodes, e.g., printers are not connected to server nodes.
Homophily-based methods would fail to classify these nodes correctly, since their labels differ from their neighbors. Further, connectivity alone does not explain the roles, since for instance the printer and database in the left part of the graph have the same degree and even their neighbors have the same degrees.
%Homophily-based methods would fail to classify these nodes correctly, since their labels differ from their neighbors. Approaches relying on the shared neighborhoods to learn similarities would be also incapable to learn similarities between printers and between databases, since they do not share neighbors. Further, connectivity alone does not explain the roles, since for instance the printer and database in the left part of the graph have the same degree and even their neighbors have the same degrees.
%Assume further, that both subnetworks appear in different parts of the graph. In this case, existing methods relying on local neighborhoods are not able to establish similarities between the printer and database nodes, respectively. Further, a distinction based on degree is not possible, as the printer and database in the left part have the same degree, but printers and databases in different parts of the graph have different degrees. The local label distributions among neighbors on the other hand provide an accurate description of how printers and databases are used in the network.
}
\label{fig:example}
%\vspace{-3ex}
\end{figure}

Though labels can be considered as another type of node attributes, there exists an important difference between labels and attributes which prevents
attribute-based embeddings to generalize well on label information. Though the attribute values of the predicted node are allowed to be used for learning
the embedding, using the node labels even in an transitive way leads to overfitting and  a bad generalization performance of the learned embedding.
 %For instance, message passing neural networks would aggregate labels in a local neighborhood by propagating labels over multiple hops through the network, such that a node could receive information about its own label via its neighbors in the training stage.
We will discuss these issues in more detail in Section \ref{sec:method} and introduce a simple baseline method.
In our new method, we aggregate labels from relevant nodes directly and thus, we can completely exclude any influence of the nodes' own labels. In a first step, we determine the relevant neighbors of a given node based on \emph{Approximate Personalized PageRank (APPR)}. Since this might be an expensive task for large graphs, we use an adaption of the highly efficient algorithm from \cite{Shun:2016:PLG:2994509.2994522}. After determining the neighborhood, we compute the label distribution within the neighborhood and classify the node based on this novel representation.
We compare our new representation to state-of-the-art graph embeddings based on several benchmark datasets for node classification.
%The key contributions of our paper can be summarized as follows:
%\bi
%\item A
%\item A novel label-based approach for semi-supervised node classification in graphs, which is able to effectively incorporate the labels of local neighborhoods to describe each node.
%, which are not necessarily \red{reflected by graph communities or structural roles. The learned embeddings can be used for node classification, as well as multiple further graph learning tasks.}
%\item We introduce corresponding models, which define local label distributions in neighborhoods of varying size based on APPR and automatically learn suitable combinations of the resulting distributions which are then embedded into a latent feature space.
%\item Methods for learning the relevant label information from a cascade of neighborhoods with increasing extension.
%\item An extensive evaluation of different model architectures and a comparison of our method with state-of-the-art methods for node embedding and semi-supervised learning on attributed and non-attributed networks.
%\ei

The remainder of the paper is structured as follows: After providing a formal problem definition for our approach in Section \ref{sec:problem_setting}, we introduce our new method in Section \ref{sec:method}, starting with a discussion on the possibility of incorporating label-based features into existing models in Section \ref{subsec:motivation}.
%Relevant background for APPR will be provided in Section \ref{sec:ppr}.
After a discussion of related work in Section \ref{sec:related_work}, the performance of our model is evaluated experimentally and compared to state-of-the-art methods in Section \ref{sec:experiments}. Finally, Section \ref{sec:conclusion} concludes the paper and proposes directions for future work.

%All related methods rely on some underlying assumption, that the labels of a node strongly depend on its structural properties in the graph and, in case of feature-based approaches, on the node attributes.

%In this paper, we propose a novel \emph{label-based approach}. As a common setting, we consider the case that no node attributes are given and that a part of the nodes in the graph has already been labeled. The main motivation for our approach is to represent the nodes not only based on the graph structure, as is the case for existing embedding methods, but to additionally leverage the rich information provided by the label distribution in the graph. We illustrate this idea with a small example in Figure \ref{fig:example}. Some existing approaches already incorporate labels during training, but to the best of our knowledge, our approach is the first to focus on modeling similarity between nodes based on local label distributions in the graph.
%Ich finde wir sollten das direkt ansprechen bevor ein Gutachter gleich sagt und was is wenn die Labels nicht bekannt sind
%Let us note that our appraoch is based on the assumption that at least a part of the neighbors of a prediciton node has already been labeled. Though this might not be the case in all applications, we argue that in the majority of applications new nodes are connected to already known parts of the network. For instance, new papers usually cite established articles and new members of a social network will usually already know multiple friends in the network to connect to.
%The learned representations may be used for a multitude of graph learning tasks. In this paper, we focus on node classification. Another interesting application might be to identify nodes with unexpected labels to detect labeling errors or outlier nodes. Furthermore, our approach generalizes to attributed networks and may be used to complement feature-based methods.

%The main idea of our approach is to learn a representation for each node, where two nodes will have similar representations, if the labels in their local neighborhoods are distributed similarly. The intuition behind this idea is to learn, how different groups, defined by labels, appear in the graph and how they depend on each other locally. Representing nodes by their local label distributions further allows for relating distant nodes in the graph, which is not possible with techniques considering the neighboring nodes themselves. It is also worth noting that the model can naturally deal with missing labels, which are simply not counted for the label distributions. In contrast to most existing methods, which define local neighborhoods via $k$-neighborhoods or samples from random walks, we employ \emph{Approximate Personalized PageRank (APPR)} to identify relevant neighbors for a given node, using an adapted, highly efficient algorithm from \cite{Shun:2016:PLG:2994509.2994522}. In order to capture patterns on multiple scales, we consider neighborhoods of increasing size by varying the teleportation parameter in PPR. For learning an optimal combination of the resulting label distributions, we propose and evaluate several model architecture alternatives.

%The rise of graph-structured data, such as social networks, communication networks, sensor networks or citation networks has lead to an increased interest in learning algorithms, which can leverage underlying graph structure to improve results on various machine learning tasks.
% Story?
% \begin{itemize}
% \item word2vec based
% \item incorporate features
% \item convolutional
% \item label information useful
% \item label distribution within neighborhoods
% \item applications
% \end{itemize}
%Based on the success of deep learning in a multitude of applications, recent activity in the field has placed a strong focus on generalizing such models to graph-structured domains.
% %representation learning and convolutional networks are especially effective
% Though recent developments have lead to major improvements, learning from graph-structured data remains a challenging problem.


==> with_comments/method_.tex <==
%!TEX root = ./main.tex

\section{Semi-supervised learning on graphs based on local label distribution}
\label{sec:method}

%\red{Julian: shortly describe what is discussed in that section; reuse some of the motivation from old section diffToConv?; appr is missing; text somewhat scarse, could have a nicer flow; some linguistic issues; another problem with label propagation: labels cannot be propagated through nodes with observed labels which impairs aggregation of labels; drop ppr to source -> pprs not normalized -> normalize after dot; overfitting: we could regularize ...; large training cost: we do not evaluate this; make motivation for shared weight matrix more clear; in general, the motivation for these different models is missing (why multiple alphas, which neighbors are important for which node, etc.); models with additional embeddings are missing; modified gcn models are missing (should appear as baselines in motivation)}
\subsection{Labels as Attributes}
\label{subsec:motivation}

The main idea of our approach is to learn a more descriptive node representation by incorporating the known labels in the neighborhood of a node. %We've discovered that it is not simple with existing methods.
In the following, we will show why existing methods  are not suitable to consider this information. Methods relying on neighborhood similarity \cite{perozzi2014deepwalk, grover2016node2vec, cao2015grarep, tang2015line,wang2016structural, faerman2017lasagne, bojchevski2017deep} learn representations in an unsupervised manner and thus, only rely on the topology of the graph and not on attributes or labels.
The \textit{Planetoid-T} model \cite{yang2016revisiting} considers labels by partly enforcing the similarity between members of the same class and therefore, nodes are related to each other based only on their own labels.
%However, Planetoid-T can only consider
%direct neighbors and does not consider the neighborhood of a node in complete.
%First steps in this direction was done by Planetoid-T model \cite{yang2016revisiting} where a higher similarity is partly enforced between nodes of particular classes and neighbors of the same class members.
%and transitively between nodes having neighbors from the same

Graph Neural Networks \cite{scarselli2009graph,li2016gated} or Graph Convolution Networks (GCN) \cite{DBLP:journals/corr/BrunaZSL13,DBLP:journals/corr/HenaffBL15, NIPS2016_6081, kipf2016semi, DBLP:journals/corr/AtwoodT15, DBLP:journals/corr/MontiBMRSB16, DBLP:journals/corr/LevieMBB17,simonovsky2017dynamic,velivckovic2017graph} are special cases of a Message Passing Neural Network (MPNN) \cite{gilmer2017neural} which is a framework describing a family of neural network based models for attributed graphs.
All MPNN methods have in common that they use some differentiable function to iteratively compute messages for each node which are passed to all its neighbors. These messages build an input to a differentiable update function which computes new node representations $h$:
$$m_{v}^{t+1} = \sum_{w\in N(v)}M_{t}(h_{v}^t,h_{w}^t),$$
$$h_{v}^{t+1} = U_{t}(h_{v}^t, m_{v}^{t+1}).$$
Here $t$ denotes the current iteration, $h_{v}^t$ is the representation of node $v$ in iteration $t$ and vector $h_{v}^0$ corresponds to the input features of node $v$. $N(v)$ denotes the set of direct neighbors of node $v$, $M_{t}$ is the message and $U_{t}$ the set of update functions.
%In the case of GCN $t$ denotes number of convolution layers and therefore size of the reception field for each node which is measured in number of hopes.
The obvious way to integrate the neighborhood label information into an MPNN-based prediction model is to include the label information into the messages directed to the neighbors in the first iteration.
However, even after removing self-links each node would receive information about its own labels already in the second iteration during the training stage. Thus, models learned on these representations overfit on the nodes' own labels and do not generalize well in the inference step where the node labels are unknown.
%In the training process it can learn that nodes label is encoded in the messages from its neighbors after the first iteration. However,
%\red{Consider for example Figure \ref{fig:example} and let us assume the problem is still to predict device types for the printer on the right side. It is unknown that the device is a printer and labels for all other devices are in the training set. Let us consider what information would the model evaluate for the printer instance in the training dataset (left printer), if one of the MPNN models is used to communicate the local label distribution. In the first iteration, the printer would get an update message with the information that all its one hop neighbors are laptops. In the second step, the update messages of the printer's neighbors would report that a printer was under their neighbors in the first iteration. However, at the inference step, where the model has to determine for the device on the right side that it is a printer, it should rely only on information about laptops and databases in its second hop neighborhood.}
The same applies to directed graphs with cycles. Therefore, applying MPNN models to communicate neighboring labels is restricted to one iteration only. We use a corresponding model as a baseline for our experiments.

Note that this problem does not apply to label propagation algorithms \cite{zhou2004learning,zhu2003semi} since they do not have separate training and inference steps.
%eine Erkl?ung warum label propagation nicht die optimale L?sung ist sollte hier schon stehen.
However, these methods have to be recomputed for predicting new objects which limits their usability.

%Each node gets a message from all its neighbors based on their last hidden state. Hidden state of the neighbors after first step already contains information about node label. Therefore node label will be encoded in each message from its neighbor in the second step. Model learned on

%$M_{1}(h_{v}^0,h_{w}^0)$ could contain $y_{w}$ label of $w$ if it is known. However, already in the next step, if graph $G$ is undirected, there is  a message $M_{2}(h_{w}^1,h_{v}^1)$ in other direction. The content of this message to node $w$ is extracted from $h_{v}^1$ and $v$ received information about label of $w$ in the previous state. Therefore the simplest thing the

\subsection{General Approach}
%Overview on the complete method
%In this section, we propose a new method for semi-supervised learning on graphs which uses local label distributions.
%Our method proceeds in two steps. We first generate a vector representing the label distribution in the local neighborhood of each node.
%In the second step, the label distribution vector is used as input to an arbitrary classification model which predicts the node labels.

% In the second step, we pass this tensor into a neural network which learns to extract the relevant information from the different local neighbors and combines them into a meaningful feature representation. Finally, the last representation layer serves as input for a classification network which can be trained jointly with the representation layer.
%highlight APPR
%To describe the local neighborhood of a node, we employ Approximated \textit{Personalized PageRank} (APPR).
%For a lot of real-world graphs, most of the nodes can be reached within a few steps. Thus, for fixed hop neighborhoods or neighbors discovered by random walks, irrelevant neighbors may absorb a significant amount of the overall probability mass as discussed in \cite{faerman2017lasagne}. In contrast, using APPR and setting the approximation parameter appropriately can ensure that only the most relevant nodes are taken into account.
%highlight the use of multiple neighnorhoods
%The locality of the explored neighborhood is controlled by the teleportation parameter $\alpha \in [0,1]$. A high teleportation probability forces to consider a local neighborhood, and vice versa, a small value for $\alpha$ typically allows a wider exploration of the node neighborhood. However, depending on the density of the local neighborhood, APPR with the same teleportation probability and approximation parameter may explore different hop neighborhoods of a node.
To present our method for semi-supervised learning on graphs using local label distributions we first outline an efficient algorithm for computing node neighborhoods based on \textit{Approximated Personalized PageRank} (APPR).
%In the following, we present our method for semi-supervised learning on graphs using local label distributions. Therefore, we outline an efficient algorithm for computing node neighborhoods based on \textit{Approximated Personalized PageRank} (APPR). 
Afterwards, we describe how to create node representations based on the label distribution in the local neighborhood based on APPR. Finally, the node representations can be used as feature descriptors in arbitrary classification models.
%The choice of a suitable teleportation parameter controlling the extend of the considered local neighborhoods often has a significant impact on the prediction quality.
%However, performing a grid search to determine a good parameter value is a time consuming task. Furthermore, for different classes varying teleportation parameters might yield the best results.
%Though this richer representation will contain irrelevant information, the subsequent processing within our network architecture can learn which of the provided information is useful for classification and which is not.
%Combining multiple local label distribution representations on graph level and training only one model avoids need for grid search. Providing multiple label distributions for each node enables the model to decide what is more important for the particular prediction.
%In following we present our method for semi-supervised learning on graphs using local label distributions. Therefore, we first show how we create node representations based on the label distribution. These node representations can be used to train various types of models.
%Second, we present different ways to feed label neighborhood representations for different locality levels into a neural network and to learn an optimal combination of label neighborhoods as part of training the neural networks.
%in various local neighborhoods.
% Each node representation is composed of multiple parts or vectors and each vector represents a label distribution in a neighborhood with a particular locality. These node representations may be used as input for various machine learning algorithms for different tasks.
%In the second part we describe our approach for efficient node-label prediction. We present different ways to feed label neighborhood representations for different locality levels into a neural network and to learn an optimal combination of label neighborhoods as part of training the neural networks.

%\subsubsection{Approximated PageRank}
%The \textit{PageRank} algorithm \cite{page1999pagerank} computes an ``importance'' score for every node in a graph. Each of the scores corresponds to the probability of a ``random surfer" to visit a node given some start distribution. The \textit{PageRank} vector is the solution of the linear system
%$pr(s) = \alpha s + (1-\alpha)pr(s)P$,
%with $P = D^{-1}A$ being the random walk transition matrix.
%$D$ is the degree matrix having the node degrees on the diagonal. The constant $\alpha$ is the \textit{teleportation} probability.
%In the following, we will describe how to compute the label distribution for a particular local neighborhood.

The \textit{Personalized PageRank} (PPR) corresponds to the \textit{PageRank} algorithm \cite{page1999pagerank}, where the probabilities in the starting vector $s$ are biased towards some set of nodes. The result is the ``importance'' of all nodes in the graph from the viewpoint of the nodes in $s$.

The \textit{push} algorithm described in \cite{jeh2003scaling} and \cite{berkhin2006bookmark} is an efficient way to compute an approximation of the \textit{Personalized PageRank} (APPR) vector if the start distribution vector $s$ is sparse.
%Note that a sparse starting vector $s$ means that a ``random surfer" may start only from a few nodes in the graph.
%The idea behind the \textit{push} algorithm is to propagate a node's probability locally and only if there is a sufficient amount of probability to update.
The idea behind the \textit{push} algorithm is only to consider a node in the local neighborhood if the probability to visit the node is significantly larger than the probability to visit any other node from the rest of the graph.
This leads to a sparse solution meaning that only relatively few nodes of the underlying graph are contained in the resulting APPR vector.

Algorithm \ref{alg:appr_ppr} describes the computation of APPR using a variant of the \textit{push} operation on lazy random walk transition matrices of undirected unweighted graphs. This algorithm was proposed in \cite{andersen2006local}, where APPR is used to partition graphs. We describe an adapted version from \cite{Shun:2016:PLG:2994509.2994522} which converges faster. %Additionally to the standard \textit{PageRank} parameters $\alpha$ and $s$, the algorithm expects the approximation parameter $\epsilon$.
The algorithm maintains two vectors: the solution vector $p$ and a residual vector $r$. The vector $p$  is the current approximation of the PPR vector and vector $r$ contains the approximation error or the not yet distributed probability mass. $p(u)$ and $r(u)$ are the entries in vectors $p$ and $r$ corresponding to node $u$, $d(u)$ is the degree of node $u$. In each iteration the algorithm selects a node with sufficient probability mass in vector $r$. This probability mass is spread  between the node entry in $p$ and the entries of its direct neighbors in $r$.
In each step, the exact PPR is the linear combination of the current solution vector $p$ and the PPR solution for $r$, i.e., $pr(s)=p+pr(r)$. This procedure can also be trivially adapted to directed graphs and graphs with weighted edges.
Moreover, the algorithm requires two parameters: $\alpha$, which is the teleportation parameter and determines the level of locality for each node neighborhood; and $\epsilon$, which is an approximation threshold and controls the approximation quality and the runtime. In fact, the \textit{push} algorithm performs updates as long as there is one node for which at least $\epsilon \frac{1-\alpha}{1+\alpha}$ probabilty mass is moved towards each of its neighbors. The complexity of the procedure is $\frac{1}{\alpha \cdot \epsilon}$.
\begin{algorithm}[t]
	\algsetup{linenosize=\fontsize{7}{8.4}}
	\fontsize{7}{8.4}
	\selectfont
	\caption{ApproximatePPR}\label{alg:appr_ppr}
	\begin{algorithmic}[1]
		\renewcommand{\algorithmicrequire}{\textbf{Input:}}
		\renewcommand{\algorithmicensure}{\textbf{Output:}}
		\REQUIRE Starting vector $s$, Teleportation probability $\alpha$, Approximation threshold $\epsilon$
		\ENSURE APPR vector $p$
		\STATE $p=\vec{0}$, $r = s$
		\WHILE {$r(u) \geq \epsilon d(u)$  for some vertex $u$}
			\STATE pick any $u$ where $r(u) \geq \epsilon d(u)$
			\STATE push(u)
		\ENDWHILE
		\RETURN $p$
		\medskip
	\end{algorithmic}
	\vspace{-1ex}
\end{algorithm}

\begin{algorithm}[t]
	\algsetup{linenosize=\fontsize{7}{8.4}}
	\fontsize{7}{8.4}
	\selectfont
	\caption{push}\label{alg:push}
	\begin{algorithmic}[1]

		\STATE $p(u) = p(u)+(2\alpha/(1+\alpha))r(u)$
		\FOR {$v$ with $(u,v)\in E$}
			\STATE $r(v) = r(v) + ((1-\alpha)/(1+\alpha))r(u)/d(u)$ \label{alg:push:line_neigh_update}
		\ENDFOR
		\STATE $r(u) = 0$%(1-\alpha)r(u)/2$
		\medskip
	\end{algorithmic}
	\vspace{-2ex}
\end{algorithm}

\subsubsection{Local Label Distribution}
In our approach we first compute the APPR vector for each node. Before APPR is computed for node $v$, the corresponding entry $s(v)$ in starting vector $s$ is set to one and all other entries to zero.
Therefore, the APPR vector of $v$ describes the importance of local neighbors only from its point of view.

In the APPR result matrix $APPR$, each row corresponds to the APPR vector of the corresponding node.
The local label distribution representation $X\in \mathbb{R}^{n \times l}$ is computed % as $X = APPR\:\mathbf{Y}_{train}$ -
by multiplying $APPR$ with the label matrix $\mathbf{Y}_{\text{\textit{train}}}$. The diagonal of $APPR$ is set to zero beforehand to exclude information about the own labels. Therefore, the entry $X_{v\:y_{j}}$ can be interpreted as the probability that a random walk starting from node $v$ stops at a neighbor with label $y_{j}$.

The local label distribution can be used as a node embedding vector which can be passed into an arbitrary classification algorithm. In our experiments, we
employ a multi-layer perceptron.

%The approximation quality and runtime are controlled by the parameter $\epsilon$. The updates are performed as long as there is a node for which at least $\epsilon \frac{1-\alpha}{(1+\alpha)d(u)}$ probability mass is moved towards each of its neighbors during the \textit{push} operation.

%\red{TODO: use notation from problem setting: aij}
%To apply Algorithm \ref{alg:appr_ppr} to directed graphs, the out degree has to be used instead of the degree.
%For weighted graphs, the update process of the neighbors has to be adapted. In the unweighted case, each neighbor gets an equal fraction of the distributed probability mass. In the weighted case, the probability mass is spread corresponding to the edge weights. Thus, line \ref{alg:push:line_neigh_update} in Algorithm \ref{alg:push} must be replaced by
%$$r(v) = r(v) + \frac{w_{u\rightarrow v}}{\sum_{i=0}^{n}w_{u\rightarrow i}}((1-\alpha)/(1+\alpha))r(u),$$
%where $n$ is the number of neighbors of $u$ and $w_{u\rightarrow v}$ denotes the weight of the edge connecting vertices $u$ and $v$.


==> with_comments/problem_setting_.tex <==
%!TEX root = ./main.tex
\section{Problem Setting}
\label{sec:problem_setting}

We consider (possibly directed) graphs $G=(V,E)$, with node set $V = \{v_1, \dots, v_n \}$ and edge set $E \subseteq V \times V$. A graph can be represented by an $n \times n$ adjacency matrix $A = (a_{ij})_{v_i,v_j \in V}$, where $a_{ij} \in \R$ denotes the weight of the edge $(v_i,v_j)$. In case of an unweighted graph,  $a_{i,j} = 1$ indicates the existence and  $a_{i,j} = 0$ the absence of an edge between $v_i$ and $v_j$. Furthermore, we do not allow self-links, i.e.,
 $a_{i,i} = 0$ for all nodes $v_i \in V$.
%For most real world graphs, the adjacency matrix is usually very sparse.
In an attributed graph, additional node attributes are provided in the form of an attribute vector $f_i \in \R^d$ for each node $v_i$. The attribute information for the whole graph can be represented by an $n \times d$ attribute matrix $F$, where the $i$th row of $F$ corresponds to $v_i$'s attribute vector $f_i$. Let us note that an important difference between attributes and labels is that attributes are usually known for all nodes, in particular those nodes without known labels.

Our problem setting is \emph{semi-supervised node classification}, where the node set $V$ is partitioned into a set of labeled nodes $L$ and unlabeled nodes $U$, such that $V = L \cup U$ and $L \cap U = \emptyset$. Thereby, each node $v_i \in V$ is associated with a label vector $y_i \in \{0, 1\}^l$, where $l$ is the number of possible labels and an entry one indicates the presence of the corresponding label for a certain node. The labels available for training can be represented by an $n \times l$ label matrix $Y_{\text{\textit{train}}}$, where the $i$'ths row of $Y_{\text{\textit{train}}}$ corresponds to the label vector $y_i$ of $v_i$ if $v_i \in L$. For unlabeled nodes, we assign constant zero vectors. The task is now to train a classifier using $A$, $Y_{\text{\textit{train}}}$ and possibly $F$ which accurately predicts $y_i$ for each $v_i \in U$. In \emph{multi-class} classification, each node is assigned to exactly one class, such that $y_i = e_j$ is the $j$'s unit vector, if $v_i$ is assigned to class $j$. \emph{Multi-label} classification denotes the general case, in which each node may be assigned to one or more classes and the goal is to predict all labels assigned to a particular node.

%In this section, we formalize our setting and provide a problem definition of the examined task. Given a graph $G=(V, E, M)$ where $V=\{v_1,\ldots,v_n\}$ denotes the set of nodes and $E \in V \times V$ describes the set of links. The $n \times n$ weight matrix $A$ denotes links weights $a_{i,j} \in \R^{+}$ for weighted graphs and $a_{i,j} \in \{0,1\}$ for unweighted. Let us note that $G$ might be directed.   Furthermore, let $C=\{c_1,\ldots,c_l\}$ be a set of class labels where $class(v_i)= y_i \in \{0,1\}^l$ describes the binary class indicator vector of node $v_i \in V$. Thus, if $v_i$ belongs to class $c_j$ than $y_{i,j}= 1$ and $y_{i,j} = 0$ otherwise.
%In our semi-supervised setting, the $n \times l$ label matrix $Y=[y_1,\ldots,y_n]^T$ is only known for at the subset of nodes $V_{train}$. Thus, $Y_{train}=\{\hat{y}_1,\ldots,\hat{y}_n\}^T$ defines the matrix of known labels where $\hat{y}_i=y_i$ if $v_i \in V_{train}$ and $\hat{y}_i = \vec{0}$ otherwise. We denote the set of all nodes $v \not \in V_{train}$ as $V_{predict}$. The task of this paper is to train a function $f(v_i)$ which predicts $y_i$ for all $v_i \in V_{predict}$.


==> with_comments/related_work_.tex <==
% !TEX root = main.tex

\section{Related Work}
\label{sec:related_work}

Numerous approaches for semi-supervised learning on graphs have been proposed in recent years. This can be sorted into two main categories, unsupervised node embedding techniques and semi-supervised techniques.
%Numerous approaches for semi-supervised learning on graphs have been proposed in recent years, which can for the most part be sorted into two categories, approaches relying solely on the graph structure (connectivity-based), and approaches considering additional node attributes (attribute-based). In this section, we would like to briefly review both of these settings and relate existing methods to our proposed approach.

\subsection{Unsupervised Node Embedding}
\label{subsec:semi_graphs}

%More formally, the goal is to learn a vector $x_i \in \R^h$ for each node $v_i$ in the graph, such that $x_i \approx x_j$ iff $\Ncal(v_i) \approx \Ncal(v_j)$, where $\Ncal(v_i)$ describes the neighborhood of node $v_i$.
%Different methods propose different neighborhood definitions, which are in most cases based on local $k$-neighborhoods or random walks. The learned node embeddings can be used as an input to various subsequent down-stream tasks, such as visualization, link prediction or node classification, and allow for the use of standard techniques operating on Euclidean data. Most existing node embedding methods define a model based on the \emph{SkipGram} architecture \cite{mikolov2013efficient, mikolov2013distributed} and train it using focus-context pairs sampled from random walks in the graph. The main idea behind these approaches is, that two nodes are similar, if they appear in similar contexts, i.e. if they can reach similar nodes with similar probabilities via random walks. \emph{DeepWalk} \cite{perozzi2014deepwalk} samples a number of first-order random walks from the graph and then samples focus-context pairs from a sliding window to train a SkipGram model. \emph{Node2vec} \cite{grover2016node2vec} attempts to capture nodes with similar structural roles in addition to community structures by sampling biased second-order random walks. \emph{LINE} \cite{tang2015line} is another variant, which considers direct first- and second-order proximities instead of random walks.
%Different methods propose different neighborhood definitions, which are in most cases based on local $k$-neighborhoods or random walks.

A strong focus of recent developments related to learning from structural relationships has been placed on learning \emph{node embeddings}, where a latent vector representation is learned for each node, reflecting its connectivity in the underlying graph. The learned node embeddings can be used as an input to a subsequent down-stream task, such as node classification.
Random walk based methods \cite{perozzi2014deepwalk,grover2016node2vec} sample a number of random walks from the graph and nodes are related if they have common neighbors. \emph{LINE} \cite{tang2015line} is another variant, which considers direct first- and second-order proximities instead of random walks. \emph{Graph2Gauss} \cite{bojchevski2017deep} learns similarity to hop neighborhoods and embeds each node as a Gaussian distribution to allow for uncertainty in the representation. \emph{GECS} \cite{al2016gecs} uses connections subgraphs to determine appropriate node neighborhood. More closely related to our approach, \emph{LASAGNE} \cite{faerman2017lasagne} relies on APPR to determine relevant context nodes. Other works perform matrix factorization. For instance, \emph{GraRep} \cite{cao2015grarep} factorizes a sequence of $k$-step log-probability matrices with SVD and concatenates the resulting low-dimensional node representations to form the final representations. Abu-El-Haija et al. propose matrix factorization of random-walk occurrence matrix with different approaches to determine context window size distribution \cite{abu2017watch}. \emph{SDNE} \cite{wang2016structural} uses a multi-layer auto-encoder model to capture non-linear structures based on direct first- and second-order proximities. Authors of \cite{chamberlain2017neural} propose embeddings in hyperbolic space. \emph{HARP} \cite{chen2017harp} addresses the local minima problem and introduce an iterative scheme for learning of node representations which can be used with different embedding learning methods. An input graph is coarsened on different levels and node representations are learned starting with the coarsest graph and learned embeddings are provided as initializations for the embeddings of subsequent finer graphs.
While the above methods rely on the homophily assumption, \emph{struc2vec} \cite{ribeiro2017struc2vec} aims at learning representations which relate structurally similar nodes instead of nodes which are close in the graph. It does so by using degree sequences in neighborhoods of different sizes.
All of the above approaches are \emph{transductive} in the sense that labels can only be predicted for unlabeled nodes observed already at training time. The \emph{GraphSAGE} \cite{hamilton2017inductive} framework introduces \emph{inductive} node embeddings. The basic idea is to learn an embedding function by sampling and aggregating node attributes in local neighborhoods. The embedding function can further be learned with a supervised loss function.  Inductive models are also obtained by considering node attributes. \emph{Variational Graph Auto-Encoders} \cite{kipf2016variational} learn node representations using a variational auto-encoder, where the encoder is a two-layer GCN. The model can be applied to attributed and non-attributed graphs.
%A more complete and recent survey of node embedding methods is provided by \cite{hamilton2017representation}.

%The main assumption underlying all of the above approaches is that two nodes should only be considered similar, if they have similar nodes appearing in their respective neighborhoods, i.e. if they are located in same graph community. This can be a severe limitation, since two nodes may also be strongly related even if they are not close in the graph. In contrast, for our approach, it is sufficient for the nodes to have similar label distributions in their neighborhoods, irrespective of the particular nodes contained in them.

%In addition to community structure, structural roles may also be important for several semi-supervised learning problems.
%Node2Vec is in principle able to capture structural similarity, but the model is somewhat limited in this regard. For instance, two nodes can only be considered structurally similar, if their geodesic distance in the graph is not larger than the size of the context window.
%The recently introduced method \emph{struc2vec} \cite{ribeiro2017struc2vec} samples random walks from a constructed multilayer graph, which encodes structural similarity between nodes based on degree sequences in neighborhoods of different sizes.
%Though struc2vec can reliably identify structurally similar nodes, it is limited to applications, in which node labels can be assumed to be defined by degree distributions in local neighborhoods. Then again, our approach is able to find related nodes, regardless of whether they have similar structural roles or appear in the same graph communities.
%Even if degree distribution in the neighborhood may bring interesting insights about graph, these representations are limited for particular supervised tasks, since different labeled communities may be similar in this context or communities with the same label may have different degree distribution.\red{remove?: Though struc2vec can reliably identify structurally similar nodes, it is limited to applications, in which node labels can be assumed to be defined by degree distributions in local neighborhoods. Then again, our approach is able to find related nodes, regardless of whether they have similar structural roles or appear in the same graph communities.}

%Similarly as the previous methods, struc2vec is only able to model a single type of node relations, which in this case is structural similarity. \red{evg: kuerzen? oder statt structural similarity degree distr of the neighbors schreiben?} Our approach however is able to find related nodes, regardless of whether they are structurally similar or appear in the same graph communities.

%Compared to separately optimizing steps in a semi-supervised learning pipeline, as is the case for semi-supervised learning with pre-trained graph embeddings, end-to-end training usually leads to better performance on the supervised learning objective. The \emph{Planetoid} framework \cite{yang2016revisiting} introduces several models for jointly learning node embeddings and predicting node labels. The main idea is to alternate between a supervised and an unsupervised loss-function during training, where contexts are sampled not only based on random walks, but additionally based on node labels. One variant of the model called \emph{Planetoid-G} considers only the graph structure, without relying on additional features. By sampling nodes with shared labels as contexts, Planetoid takes a first step in the direction of incorporating label information. However, nodes are only related to each other based on their own labels, whereas local label distributions are significantly more informative, as our experiments show.

\subsection{Semi-Supervised Learning on Graphs}

Compared to separately optimizing steps in a semi-supervised learning pipeline, as is the case for semi-supervised learning with pre-trained node embeddings, end-to-end training usually leads to better performance on the supervised learning objective.

%In addition to related work on learning based on graph structure, there exists a large body of related approaches primarily specializing in incorporating additional node attributes to improve semi-supervised learning on graphs. In this setting, each node $v_i$ in the graph is associated with a feature vector $x_i \in \R^d$, providing additional information about the entity modeled by the respective node, which is not contained in the graph structure.
%The feature vectors of all nodes in the graph can be aggregated in a feature matrix $X \in \R^{n \times d}$.
%In general, all of the related approaches in this setting are different from our approach in that they focus on node attributes, where our approach focuses on local label distributions and can also be applied to non-attributed graphs. Even in this setting, our approach is still able to outperform some of the related methods, as demonstrated in our experiments.

%One important direction in this setting is Laplacian Regularization, where a supervised loss function based on the input features is augmented with an unsupervised loss function based on the graph's Laplacian matrix, encoding the assumption that close-by nodes should have the same label. Related approaches include for instance \emph{Label Propagation} \cite{zhu2003semi} and \emph{Manifold Regularization} \cite{belkin2006manifold}. \emph{Deep Semi-Supervised Embedding} \cite{weston2012deep} further incorporates node embeddings by augmenting neural network models with an embedding layer.
One important direction is \emph{Laplacian Regularization}, where the prediction loss is augmented with an unsupervised loss function based on the graph's Laplacian matrix, encoding the homophily assumption that close-by nodes should have the same label. Related approaches include \emph{Manifold Regularization} \cite{belkin2006manifold}, a kernel-based method, and \emph{Deep Semi-Supervised Embedding} \cite{weston2012deep} which incorporates node embeddings by augmenting neural network models with an embedding layer. Both of these methods generalize to attributed graphs. \emph{Label Propagation} \cite{zhu2003semi, zhou2004learning} is more closely related to our approach. The main idea is to propagate the observed labels through the graph via the random walk transition matrix. Similarly, \emph{Collective Classification} \cite{sen2008collective} starts with the observed labels and iteratively classifies nodes based on previously inferred labels in the local neighborhood based on a majority vote. However, none of these two methods considers additional node attributes and no actual learning is involved. Similarly to collective classification, the more recent methods \emph{Structural Neighborhood Based Classification} \cite{nandanwar2016structural} and \emph{Weighted-Vote Geometric Neighbor Classification} \cite{ye2017learning} also classify nodes based on labels in local neighborhoods. They achieve this by learning a model which predicts node labels from a feature vector describing the local $k$-neighborhood. Both methods assume an unattributed graph.

Instead of imposing regularization, \emph{Planetoid} \cite{yang2016revisiting} combines the prediction loss with node embeddings by training a joint model which predicts class labels as well as graph context for a given node. The graph context sampled from random walks as well as the set of nodes with shared labels. This allows Planetoid to relate nodes with similar labels even if they are not close in the graph. Thus, Planetoid does not rely on a strong homophily assumption. In addition to a connectivity-based variant, \emph{Planetoid-G}, the authors propose two further architectures, which incorporate node attributes. The transductive variant \emph{Planetoid-T} starts with pre-trained embeddings and alternately optimizes the prediction and embedding loss functions. The inductive variant \emph{Planetoid-I} on the other hand predicts the graph context from the node features instead.

Another important direction which has recently gained increasing attention is concerned with generalizing deep neural network architectures to graph-structured domains.
%As these models are most closely related to our approach, we will discuss them separately in Section \ref{sec:diff_to_conv} and distinguish them from our approach.
As the general approach consists of incorporating graph structure into supervised learning, these models assume an attributed graph. However, they can naturally be applied to non-attributed graphs by using the identity matrix as the attribute matrix. The vast majority of neural network based models for semi-supervised learning on graphs can be described within a message-passing framework. In a \emph{Message Passing Neural Network (MPNN)} \cite{gilmer2017neural}, each node has a hidden state which is updated iteratively during training. The initial hidden state of a node corresponds to it's attribute vector. In a first step, messages from $v_i$'s neighborhood are received and aggregated, where a message from neighbor $v_j$ depends on $v_i$'s and $v_j$'s hidden states. In a second step, $v_i$'s state is updated by combining it with the aggregated messages.
%Two important special cases of this framework are Graph Neural Networks and Graph Convolution Networks.
%In \emph{Graph Neural Networks} \cite{scarselli2009graph, li2016gated},
%\red{TODO: main idea? what are the two phases in message passing?}
An important special case are \emph{Graph Convolution Networks} \cite{DBLP:journals/corr/BrunaZSL13, DBLP:journals/corr/HenaffBL15, NIPS2016_6081, kipf2016semi,  DBLP:journals/corr/MontiBMRSB16, DBLP:journals/corr/LevieMBB17, velivckovic2017graph}
which aggregate node attributes over local neighborhoods with spatially localized filters, similar to classical convolutional networks on images \cite{lecun1989backpropagation}. The \emph{ChebNet} \cite{NIPS2016_6081} aggregates messages from neighbors analogously to the eigenvectors of the graph's Laplacian matrix. The update function ignores the previous state and applies a non-linear activation. The resulting filters are $k$-localized. The \emph{GCN} \cite{kipf2016semi} is a simplification of the ChebNet, which only considers one-hop neighbors. Messages are aggregated according to a normalized adjacency matrix. In the update phase, the aggregated messages are multiplied with a learned filter matrix with a ReLU activation. For graph convolution networks, the number of message passing iterations corresponds to the number of layers.
%The \emph{FastGCN} \cite{chen2018fastgcn} is a variant of the GCN which considers only a part of the neighborhood for each node.
%\emph{Graph Attention Networks} \cite{velivckovic2017graph} use an attention mechanism to decide which of the incoming messages are most important.
%The \emph{GCNTD} model \cite{chen2017graph} uses external information about the structure of the label space, e.g. "a husky is a mammal".


%\red{comment: conv on graphs are more general, e.g. diffusion networks. How important is signal processing, not another name for features? what about just point to conv comp section?
%Another important direction, which has recently gained increasing attention, considers signal processing on graphs \cite{shuman2013emerging} to perform semi-supervised learning. In this field, the feature matrix of the graph is interpreted as a signal on the graph nodes and main research questions are concerned with generalizing analysis of classic discrete-time signals to graph signals. This theory can be used to generalize convolutional networks to graphs. As these models are most closely related to our approach, we will discuss them separately in Section \ref{sec:diff_to_conv} and distinguish them from our approach.}

% An important tool is the Graph Fourier Transform, which can be used to formulate a spectral convolution operator for graphs. This is implemented by Spectral CNNs \cite{DBLP:journals/corr/HenaffBL15}, but they suffer from high training time and the learned filters are not localized in the vertex domain. -> not here, discuss in diff_to_conv section
%especially graph convolution: bruna \cite{DBLP:journals/corr/HenaffBL15}, defferard \cite{NIPS2016_6081}, kipf \cite{kipf2016semi}, geometric deep learning survey
%- in Section \ref{sec:diff_to_conv}, we will discuss graph convolutional networks in more detail and distinguish them from our proposed approach

